Accelerated Decentralized Stochastic Gradient Descent for Strongly Convex Optimization

Decentralized stochastic optimization is a fundamental paradigm for large-scale learning over networks, where agents communicate only with their neighbors and no central coordinator is required. For strongly convex problems, communication efficiency is mainly determined by the condition number \(\kappa=L/\mu\) and the network spectral gap \(1-\beta\). Although deterministic decentralized methods can simultaneously achieve accelerated \(\sqrt{\kappa}\) and \(1/\sqrt{1-\beta}\) dependences, no existing stochastic method attains both improvements at once. In this paper, we propose \emph{Multi-Gossip Accelerated DSGD} (MG-ADSGD), a decentralized stochastic algorithm that combines Nesterov-type primal--dual extrapolation with multi-round fast gossip averaging. The key idea is to couple the gossip depth with the mini-batch size so that additional communication rounds simultaneously improve consensus accuracy and reduce gradient variance. We show that MG-ADSGD achieves the communication complexity \[ \widetilde{\mathcal O}\!\left( \frac{\sigma^2}{\mu n\epsilon}\log\frac{1}{\epsilon} + \sqrt{\frac{\kappa}{1-\beta}}\log\frac{1}{\epsilon} \right), \] where \(\epsilon\) denotes the target accuracy, \(n\) is the number of nodes, and \(\sigma^2\) is the gradient variance. To the best of our knowledge, this bound yields the best currently available communication complexity for decentralized stochastic strongly convex optimization, up to logarithmic factors that are independent of $\epsilon$.

==> experiments.tex <==
\section{Experiment Design}
\label{sec:experiments}

This section presents the planned empirical study for \emph{Multi-Gossip Accelerated DSGD}. As requested, we do not run experiments in the current draft; instead, we provide a detailed and executable evaluation blueprint aligned with the algorithmic design and the current theory. The main purpose of the experiments is to test the communication advantages of the proposed method, identify when multiple accelerated gossip rounds are beneficial, and check whether the observed trends are consistent with the predicted dependence on the stochastic variance, condition number, and network connectivity.

\subsection{Experimental goals}
We propose to answer the following questions.
\begin{enumerate}
    \item Does \emph{Multi-Gossip Accelerated DSGD} reduce the number of communication rounds required to reach a target accuracy compared with single-gossip decentralized stochastic methods?
    \item How much of the improvement comes from the accelerated optimization structure, and how much comes from the accelerated multi-gossip communication primitive?
    \item How does the preferred gossip depth $R$ vary with the graph spectral gap $1-\beta$, the condition number $L/\mu$, and the stochastic noise level?
    \item In homogeneous-optimum settings, does the measured communication complexity behave consistently with the theorem-guided scaling
    \[
    \widetilde{\mathcal O}\!\left(
    \frac{\sigma^2}{\mu n\epsilon}
    +
    \sqrt{\frac{L}{\mu}}\frac{1}{\sqrt{1-\beta}}
    \right)
    \]
    up to logarithmic factors?
    \item In heterogeneous-optimum settings, how visible is the additional residual effect associated with the quantity $G^\ast$?
\end{enumerate}

\subsection{Benchmark suite}
We propose three benchmark families.

\paragraph{(A) Synthetic strongly convex quadratics.}
This is the primary benchmark family because it matches the theory most closely and allows direct control of all key parameters. At node $i$, we define
\[
f_i(x)=\frac{1}{2}(x-a_i)^\top H_i(x-a_i),
\]
where $H_i\in\mathbb R^{d\times d}$ is positive definite with eigenvalues in $[\mu,L]$. We suggest using dimensions $d\in\{20,100,500\}$ and numbers of nodes $n\in\{8,16,32\}$.

We propose two synthetic regimes.
\begin{itemize}
    \item \textbf{Homogeneous-optimum case:} choose all local minimizers equal, e.g., $a_i=a^\star$ for every $i$. Then $x^\star=a^\star$ and the setting is consistent with $G^\ast=0$.
    \item \textbf{Heterogeneous-optimum case:} choose $a_i=a^\star+b_i$ with nonzero local shifts $b_i$ satisfying $\sum_i b_i=0$. This keeps the global optimum controlled while generating nonzero local gradients at $x^\star$.
\end{itemize}

To model stochastic gradients, node $i$ returns
\[
\nabla F_i(x;\xi)=H_i(x-a_i)+\zeta_i,
\]
where $\zeta_i$ is zero-mean noise with covariance chosen to realize prescribed variance levels. We recommend testing noise scales corresponding to low, medium, and high variance, for example $\sigma\in\{10^{-3},10^{-2},10^{-1}\}$ after normalization.

\paragraph{(B) Strongly convex empirical-risk minimization.}
To move beyond synthetic problems while preserving strong convexity, we propose two standard regularized models.
\begin{itemize}
    \item \textbf{Ridge regression:}
    \[
    f_i(x)=\frac{1}{m_i}\sum_{j=1}^{m_i}\frac12(\langle a_{ij},x\rangle-b_{ij})^2+\frac{\lambda}{2}\|x\|^2.
    \]
    \item \textbf{$\ell_2$-regularized logistic regression:}
    \[
    f_i(x)=\frac{1}{m_i}\sum_{j=1}^{m_i}\log\bigl(1+\exp(-b_{ij}\langle a_{ij},x\rangle)\bigr)+\frac{\lambda}{2}\|x\|^2.
    \]
\end{itemize}
Candidate datasets include a9a, ijcnn1, w8a, and binary-classification versions of MNIST or Fashion-MNIST after standard preprocessing. Data should be partitioned across nodes in two ways:
\begin{itemize}
    \item \textbf{i.i.d. split:} to approximate the homogeneous setting;
    \item \textbf{label-skew or feature-skew split:} to create heterogeneous local objectives.
\end{itemize}
The regularization parameter $\lambda$ should be chosen so that the effective objective is strongly convex and the smoothness and strong-convexity constants are numerically estimable.

\paragraph{(C) Network stress tests.}
To isolate communication effects, we propose fixing the optimization problem and varying only the communication topology. Recommended graph families are:
\begin{itemize}
    \item ring,
    \item 2D grid,
    \item random geometric graph,
    \item Erd\H{o}s--R\'enyi sparse graph conditioned on connectivity,
    \item expander-like sparse graph.
\end{itemize}
For each graph, the communication matrix should be symmetric and doubly stochastic, for example using Metropolis weights. The second-largest eigenvalue should be estimated numerically so that each topology can be annotated by its effective spectral gap parameter.

\subsection{Baselines and ablations}
The proposed method should be compared with the following baselines.
\begin{itemize}
    \item \textbf{D-SGD / D-PSGD:} decentralized stochastic gradient descent with one mixing step per outer iteration.
    \item \textbf{Multi-consensus DSGD:} same outer-iteration structure and same communication budget, but replace accelerated gossip by $R$ rounds of ordinary consensus.
    \item \textbf{No optimization acceleration:} keep the same multi-gossip communication primitive but remove the extrapolated $(x,z,y)$ accelerated structure.
    \item \textbf{No communication acceleration:} keep the accelerated optimization structure but replace FGA with standard repeated mixing.
    \item \textbf{A bias-corrected strongly-convex baseline:} exact diffusion, EXTRA-type stochastic variant, or a representative gradient-tracking method, depending on implementation availability.
\end{itemize}

The two most important ablations are:
\begin{enumerate}
    \item proposed method versus D-SGD, to test communication efficiency against the standard baseline;
    \item proposed method versus non-accelerated multi-consensus, to isolate the benefit of accelerated gossip.
\end{enumerate}

\subsection{Communication and oracle budgets}
Each method should be evaluated under two complementary x-axes.
\begin{enumerate}
    \item \textbf{Total communication rounds.} This is the main axis for validating the theory.
    \item \textbf{Total stochastic-gradient evaluations.} This controls for the fact that in the proposed method the batch size satisfies $B=R$.
\end{enumerate}
For the proposed algorithm, if one outer iteration uses $R$ gossip rounds inside the $z$-update and another $R$ gossip rounds inside the $x$-update, then the paper should clearly state whether one reports:
\begin{itemize}
    \item total edge-wise message-passing rounds, or
    \item effective communication rounds normalized per FGA call.
\end{itemize}
Whichever convention is adopted must be used consistently across all methods.

\subsection{Tuning protocol}
For \emph{Multi-Gossip Accelerated DSGD}, the initial hyperparameter grid should be driven by the theorem:
\[
\gamma\in\left\{\frac{1}{16L},\frac{1}{12L},\frac{1}{8L}\right\},
\qquad
R\in\{1,2,4,8,16\},
\qquad
\theta=\sqrt{\frac{\mu\gamma}{2}}.
\]
On graphs with very poor connectivity, an extended grid such as $R\in\{1,2,4,8,16,32\}$ may be useful.

For D-SGD and other baselines, stepsizes should be tuned over a logarithmic grid centered around their natural theoretical scale. For example, one may use
\[
\eta\in\left\{\frac{1}{L},\frac{1}{2L},\frac{1}{4L},\frac{1}{8L},\frac{1}{16L}\right\}
\]
or the analogous network-corrected scale if a baseline requires it. To avoid overfitting to one metric, hyperparameters should be selected using a validation criterion fixed in advance, such as the best objective gap at a predefined communication budget.

\subsection{Evaluation metrics}
The following quantities should be reported.
\begin{itemize}
    \item \textbf{Objective gap:} $f(\bar x^{(k)})-f^\star$.
    \item \textbf{Distance to optimum:} $\|\bar x^{(k)}-x^\star\|^2$ when $x^\star$ is available or accurately approximated.
    \item \textbf{Consensus error:} $\|\Pi x^{(k)}\|_F^2$ and, when helpful, $\|\Pi z^{(k)}\|_F^2$.
    \item \textbf{Target-accuracy communication complexity:} the number of communication rounds required to achieve each target tolerance $\epsilon$ in a prescribed list.
    \item \textbf{Stability region:} whether a method remains stable for aggressive stepsizes and low-connectivity graphs.
\end{itemize}
For synthetic quadratics, it is also useful to report the decomposition between optimization progress and consensus error, because the current proof explicitly couples these two effects.

\subsection{Core experimental matrix}
To keep the study focused, we recommend the following core matrix.
\begin{enumerate}
    \item \textbf{Quadratic / homogeneous optimum / varying topology.}
    This is the cleanest test of the communication-complexity claim under $G^\ast=0$.
    \item \textbf{Quadratic / heterogeneous optimum / varying heterogeneity level.}
    This tests the practical impact of the extra residual term associated with local mismatch.
    \item \textbf{Regularized logistic regression / i.i.d. partition / varying $R$.}
    This checks whether the communication advantage persists on a realistic learning task.
    \item \textbf{Regularized logistic regression / non-i.i.d. partition / varying topology.}
    This tests robustness under simultaneously difficult optimization and communication conditions.
\end{enumerate}

\subsection{Ablation studies}
The following ablations are central.

\paragraph{Varying gossip depth $R$.}
This ablation studies the trade-off between faster consensus and heavier communication per outer iteration. The theory suggests that increasing $R$ should improve performance on poorly connected graphs until the disagreement term is no longer dominant; after that, the gains should saturate.

\paragraph{Varying topology / spectral gap.}
At fixed optimization problem, the preferred $R$ should increase as the graph becomes less connected. This is the main experiment for testing the scaling
\[
R=\widetilde{\mathcal O}\!\left(\frac{1}{\sqrt{1-\beta}}\right).
\]
A practical implementation of this test is to compare the best communication complexity achieved by each method on ring, grid, random geometric, and expander-like graphs.

\paragraph{Homogeneous versus heterogeneous optimum.}
This ablation directly tests the role of $G^\ast$. The homogeneous setting should show the clearest agreement with the final communication-complexity theorem, whereas the heterogeneous setting should exhibit a larger residual floor.

\paragraph{Condition number and noise level.}
By varying $L/\mu$ and the gradient-noise variance, one can test whether ill-conditioning primarily affects the transient rate while noise primarily affects the final accuracy floor and the communication needed to reach small $\epsilon$.

\subsection{Expected outcomes}
The expected outcomes are:
\begin{itemize}
    \item On poorly connected graphs, the proposed method should require fewer communication rounds than D-SGD to reach a fixed objective tolerance.
    \item Accelerated gossip should outperform plain repeated consensus most clearly when the spectral gap is small.
    \item The accelerated optimization structure should improve the transient regime, especially on ill-conditioned strongly convex problems.
    \item The benefit of increasing $R$ should saturate, producing an empirically optimal intermediate gossip depth.
    \item In homogeneous-optimum problems, the measured communication complexity should be broadly consistent with the predicted separation between a stochastic term and a network term.
\end{itemize}

\subsection{Planned figures and tables}
Once experiments are run, the main paper should include at least the following figures.
\begin{enumerate}
    \item Objective gap versus communication rounds on homogeneous strongly convex quadratics.
    \item Objective gap versus communication rounds on heterogeneous strongly convex quadratics.
    \item Objective gap versus communication rounds on regularized logistic regression.
    \item Consensus error versus communication rounds for several values of $R$.
    \item Target-accuracy communication complexity versus graph family or spectral gap.
\end{enumerate}
We also recommend a table reporting the best-tuned hyperparameters for each method and benchmark, and a second table summarizing the communication rounds needed to reach several target tolerances.

\subsection{Implementation details to be fixed before execution}
Before actual experiment execution, the following implementation choices should be fixed and documented.
\begin{itemize}
    \item The exact definition of one communication round for FGA-based methods.
    \item The random seeds and number of independent trials, e.g., $5$ seeds for synthetic tasks and $3$ seeds for larger real-data tasks.
    \item The stopping criteria and maximum communication budget.
    \item The procedure used to estimate or upper-bound $(L,\mu)$ for theorem-guided tuning.
    \item The precise data partition protocol for the non-i.i.d. setting.
\end{itemize}

At the current stage, this section should be read as a concrete experiment plan rather than a results section. It is already detailed enough to support a later implementation phase without changing the scientific scope of the paper.

